Rational Deployment of Multiple Heuristics in IDA*

Recent advances in metareasoning for search has shown its usefulness in improving numerous search algorithms. This paper applies rational metareasoning to IDA* when several admissible heuristics are available. The obvious basic approach of taking the maximum of the heuristics is improved upon by lazy evaluation of the heuristics, resulting in a variant known as Lazy IDA*. We introduce a rational version of lazy IDA* that decides whether to compute the more expensive heuristics or to bypass it, based on a myopic expected regret estimate. Empirical evaluation in several domains supports the theoretical results, and shows that rational lazy IDA* is a state-of-the-art heuristic combination method.

==> Makefile <==
%.pdf: %.tex
	pdflatex $<
	bibtex `echo $< | sed 's/\.tex//'`
	pdflatex $<

all: paper.pdf b1.pdf

clean:
	rm -f paper.pdf *.aux *.bbl *.blg *.log

